Triangular flow in hydrodynamics and transport theory

In ultrarelativistic heavy-ion collisions, the Fourier decomposition of the relative azimuthal angle, \Delta \phi, distribution of particle pairs yields a large cos(3\Delta \phi) component, extending out to large rapidity separations \Delta \eta >1. This component captures a significant portion of the ridge and shoulder structures in the \Delta \phi distribution, which have been observed after contributions from elliptic flow are subtracted. An average finite triangularity due to event-by-event fluctuations in the initial matter distribution, followed by collective flow, naturally produces a cos(3\Delta \phi) correlation. Using ideal and viscous hydrodynamics, and transport theory, we study the physics of triangular (v_3) flow in comparison to elliptic (v_2), quadrangular (v_4) and pentagonal (v_5) flow. We make quantitative predictions for v_3 at RHIC and LHC as a function of centrality and transverse momentum. Our results for the centrality dependence of v_3 show a quantitative agreement with data extracted from previous correlation measurements by the STAR collaboration. This study supports previous results on the importance of triangular flow in the understanding of ridge and shoulder structures. Triangular flow is found to be a sensitive probe of initial geometry fluctuations and viscosity.

==> fig10/gnufig10 <==
set term post color eps enhan "Times-Roman" 15
set size 0.5
#set key 0.18,0.14
set style line 1 lt 1 lw 3
set style line 2 lt 2 lw 3
set style line 3 lt 3 lw 3
set style line 4 lt 4 lw 3
set style line 5 lt 5 lw 3
set style line 6 lt 6 lw 3
set style line 7 lt 7 lw 3
set style line 8 lt 8 lw 3
set style line 9 lt 9 lw 3
set style line 10 lt 10 lw 3
set style line 11 lt 9 pt 4 ps 0.7
set style line 12 lt 9 pt 5 ps 0.7
set style line 13 lt 9 pt 8 ps 0.7
set style line 14 lt 9 pt 9 ps 0.7
eps3c(x)=ac3+cc3/sqrt(x+bc3**2)
fit eps3c(x) 'AuAu-200GeVMCKLN' u ($2):($5) via ac3,bc3,cc3
eps3(x)=a3+c3/sqrt(x+b3**2)
fit eps3(x) 'EccCorr24-RHIC-x0145.dat' u ($2):($5) via a3,b3,c3
set xtics 100
set mxtics 2
set key bottom right
set xlabel "N_{Part}"
set ylabel "v_3"
set output "v3STAR.eps"
plot [*:*] [0:*] 'ptcutRHICGlauberangle0.54pisv08.dat' \
			u 2:($14*eps3($2)/$5) w l ls 2 t '{/Symbol h}/s=0.08', \
		'ptcutRHICCGCpreresoangle0.54pisv08.dat' \
                        u 2:($14*0.75*eps3c($2)/$5) w l ls 3 t '{/Symbol h}/s=0.16', \
		'STAR.dat' \
			u 1:(sqrt($4)):(sqrt($4-$5)):(sqrt($4+$5)) w yerrorbars ls 12 t 'STAR'
#plot [*:*] [0:*] 'ptcutRHICGlauberangle0.54pisv08.dat' \
#			u 2:($14*eps3($2)/$5) w l ls 2 t '{/Symbol h}/s=0.08', \
#		'ptcutRHICCGCpreresoangle0.54pisv08.dat' \
#                        u 2:($14*0.75*eps3c($2)/$5) w l ls 3 t '{/Symbol h}/s=0.16', \
#		'STAR.dat' \
#			u 1:(sqrt($4)):(sqrt($4-$5)):(sqrt($4+$5)) w yerrorbars ls 12 t 'STAR'



==> fig11/gnufig11 <==
set term post color eps enhan "Times-Roman" 15
set size 0.5
set key top left
#set data style line
set output "v3_vs_pt.eps"
set ylabel "v_3"
set label 1 '{/Symbol h}/s=0.08' at 2.1,0.060
set label 2 '{/Symbol h}/s=0.16' at 1.8,0.03
set ytics 0.02
plot [*:3.0] [-0.00:*]\
	'GlauberCentralpreresopisvall.dat' \
		u 1:($5*0.094888/0.084216) w l lt 1 lw 3 t 'pions', \
        'GlauberCentralpreresoKsvall.dat' \
                u 1:($5*0.094888/0.084216) w l lt 2 lw 3 t 'kaons', \
        'GlauberCentralpreresopsvall.dat' \
                u 1:($5*0.094888/0.084216) w l lt 3 lw 3 t 'protons', \
	'CGCCentralpreresopisvall.dat' \
		u 1:($5*0.085059/0.0841877) w l lt 1 lw 3 notitle, \
        'CGCCentralpreresoKsvall.dat' \
                u 1:($5*0.085059/0.0841877) w l lt 2 lw 3 notitle, \
        'CGCCentralpreresopsvall.dat' \
                u 1:($5*0.085059/0.0841877) w l lt 3 lw 3 notitle

==> fig11/gnuresonance <==
# plots results after resonance feeddown for Glauber
set term post color eps enhan "Times-Roman" 15
set size 0.5
#set key 0.8,1.8
set key top left
#set data style line
set output "v3_vs_pt_feeddown.eps"
set ylabel "v_3"
set label 1 '{/Symbol h}/s=0.08' at 2.1,0.060
set label 2 '{/Symbol h}/s=0.16' at 1.8,0.03
set ytics 0.02
plot [*:3.0] [-0.00:*]\
	'GlauberCentralpisvall.dat' \
		u 1:($5*0.094888/0.084216) w l lt 1 lw 3 t 'pions', \
        'GlauberCentralKsvall.dat' \
                u 1:($5*0.094888/0.084216) w l lt 2 lw 3 t 'kaons', \
        'GlauberCentralpsvall.dat' \
                u 1:($5*0.094888/0.084216) w l lt 3 lw 3 t 'protons', \
	'CGCCentralpreresopisvall.dat' \
		u 1:($5*0.085059/0.0841877) w l lt 1 lw 3 notitle, \
        'CGCCentralpreresoKsvall.dat' \
                u 1:($5*0.085059/0.0841877) w l lt 2 lw 3 notitle, \
        'CGCCentralpreresopsvall.dat' \
                u 1:($5*0.085059/0.0841877) w l lt 3 lw 3 notitle

==> fig12/gnufig12 <==
set term post color eps enhan "Times-Roman" 15
set size 0.5
set key bottom left
#set data style line
set output "v5_vs_pt.eps"
set xlabel "p_t [GeV/c]"
set ylabel "v_5"
set label 1 '{/Symbol h}/s=0.08' at 1.2,0.03
set label 2 '{/Symbol h}/s=0.16' at 2.2,0.005
set ytics 0.02
plot [0:3.0] [-0.04:0.04]\
	'v5Glauberpreresopis.dat' \
		u 1:($2*0.091425/0.080335) w l lt 1 lw 3 t 'pions', \
        'v5GlauberpreresoKs.dat' \
                u 1:($2*0.091425/0.080335) w l lt 2 lw 3 t 'kaons', \
        'v5Glauberpreresops.dat' \
                u 1:($2*0.091425/0.080335) w l lt 3 lw 3 t 'protons', \
	'v5CGCpreresopis.dat' \
		u 1:($2*0.074433/0.082867) w l lt 1 lw 3 notitle, \
        'v5CGCpreresoKs.dat' \
                u 1:($2*0.074433/0.082867) w l lt 2 lw 3 notitle, \
        'v5CGCpreresops.dat' \
                u 1:($2*0.074433/0.082867) w l lt 3 lw 3 notitle

==> fig8/gnufig8 <==
set term post color eps enhan "Times-Roman" 15
set size 0.5
set style line 1 lt 1 lw 3
set style line 2 lt 2 lw 3
set style line 3 lt 3 lw 3
set style line 4 lt 4 lw 3
set style line 5 lt 5 lw 3
set style line 6 lt 6 lw 3
set style line 7 lt 7 lw 3
set style line 8 lt 8 lw 3
set style line 9 lt 9 lw 3
set style line 10 lt 10 lw 3
set style line 11 lt 9 pt 4 ps 0.7
set style line 12 lt 9 pt 5 ps 0.7
set style line 13 lt 9 pt 8 ps 0.7
set style line 14 lt 9 pt 9 ps 0.7
set xtics 100
set mxtics 2
set key bottom right
epsc3(x)=ac3+cc3/sqrt(x+bc3**2)
fit epsc3(x) 'AuAu-200GeVMCKLN' u ($2):($5) via ac3,bc3,cc3
epsp3(x)=ap3+cp3/sqrt(x+bp3**2)
fit epsp3(x) 'PbPb-5500GeVMCKLN' u ($2):($5) via ap3,bp3,cp3
eps3(x)=a3+c3/sqrt(x+b3**2)
fit eps3(x) 'EccCorr24-RHIC-x0145.dat' u ($2):($5) via a3,b3,c3
epsh3(x)=ah3+ch3/sqrt(x+bh3**2)
fit epsh3(x) 'EccCorr24-LHC-x18.dat' u ($2):($5) via ah3,bh3,ch3
set output "v3vsNpart.eps"
set xlabel "N_{Part}"
set ylabel "v_3"
plot [0:*] [-0.001:0.025]\
		'LHCGlauberangle0.54pisv08.dat' \
			u 2:($14*epsh3($2)/$5) w l ls 4 t 'LHC, {/Symbol h}/s=0.08', \
		 'RHICGlauberangle0.54pisv08.dat' \
			u 2:($14*eps3($2)/$5) w l ls 2 t 'RHIC, {/Symbol h}/s=0.08', \
		'LHCCGCpreresoangle0.26pisv08.dat' \
			u 2:($14*0.83*epsp3($2)/$5) w l ls 5 t 'LHC, {/Symbol h}/s=0.16', \
		'RHICCGCpreresoangle0.54pisv08.dat' \
			u 2:($14*0.75*epsc3($2)/$5) w l ls 3 t 'RHIC, {/Symbol h}/s=0.16'
print eps3(352.241448)
print epsc3(352.241448)


==> fig9/gnufig9 <==
set term post color eps enhan "Times-Roman" 15
set size 0.5
#set key 0.18,0.14
set style line 1 lt 1 lw 4
set style line 2 lt 2 lw 4
set style line 3 lt 3 lw 4
set style line 4 lt 4 lw 4
set style line 5 lt 5 lw 4
set style line 6 lt 6 lw 4
set style line 7 lt 7 lw 4
set style line 8 lt 8 lw 4
set style line 9 lt 9 lw 4
set style line 10 lt 10 lw 4
set style line 11 lt 9 pt 4 ps 0.7
set style line 12 lt 9 pt 5 ps 0.7
set style line 13 lt 9 pt 8 ps 0.7
set style line 14 lt 9 pt 9 ps 0.7
set xtics 100
set mxtics 2
set key bottom right
set output 'v2STAR.eps'
set ylabel 'v_2'
set xlabel 'N_{Part}'
set key top right
#set key 300,-0.01
err=0.004
eps2c(x)=ac2-dc2*x+cc2/sqrt(x+bc2**2)
fit eps2c(x) 'AuAu-200GeVMCKLN' u ($2):($4) via ac2,bc2,cc2,dc2
eps2(x)=a2-d2*x+c2/sqrt(x+b2**2)
fit eps2(x) 'EccCorr24-RHIC-x0145.dat' u ($2):($4) via a2,b2,c2,d2
plot [*:*] [-0.00:0.2]\
		 'Glauberptcut.dat' \
			u 2:($13*eps2($2)/$7) w l ls 2 t 'Glauber', \
		'CGCptcut.dat' \
			u 2:($13*eps2c($2)/$7) w l ls 3 t 'CGC', \
                'STAR.dat' \
			u 1:(sqrt($2)):($3/2/sqrt($2)) w yerrorbars ls 12 t 'STAR'

#plot [*:*] [-0.00:0.2]\
#		 'Glauberptcut.dat' \
#			u 2:($13*eps2($2)/$7) w l ls 2 t 'Glauber (scaled)', \
#		'CGCptcut.dat' \
#			u 2:($13*eps2c($2)/$7) w l ls 3 t 'CGC (scaled)', \
#		 'Glauberptcut.dat' \
#			u 2:($13) w l lt 2 lw 1 t 'Glauber', \
#		'CGCptcut.dat' \
#			u 2:($13) w l lt 3 lw 1 t 'CGC', \
#                'STAR.dat' \
#			u 1:(sqrt($2)):($3/2/sqrt($2)) w yerrorbars ls 12 t 'STAR'


